A Survey on Mobile Edge Computing for Video Streaming: Opportunities and Challenges

5G communication brings substantial improvements in the quality of service provided to various applications by achieving higher throughput and lower latency. However, interactive multimedia applications (e.g., ultra high definition video conferencing, 3D and multiview video streaming, crowd-sourced video streaming, cloud gaming, virtual and augmented reality) are becoming more ambitious with high volume and low latency video streams putting strict demands on the already congested networks. Mobile Edge Computing (MEC) is an emerging paradigm that extends cloud computing capabilities to the edge of the network i.e., at the base station level. To meet the latency requirements and avoid the end-to-end communication with remote cloud data centers, MEC allows to store and process video content (e.g., caching, transcoding, pre-processing) at the base stations. Both video on demand and live video streaming can utilize MEC to improve existing services and develop novel use cases, such as video analytics, and targeted advertisements. MEC is expected to reshape the future of video streaming by providing ultra-reliable and low latency streaming (e.g., in augmented reality, virtual reality, and autonomous vehicles), pervasive computing (e.g., in real-time video analytics), and blockchain-enabled architecture for secure live streaming. This paper presents a comprehensive survey of recent developments in MEC-enabled video streaming bringing unprecedented improvement to enable novel use cases. A detailed review of the state-of-the-art is presented covering novel caching schemes, optimal computation offloading, cooperative caching and offloading and the use of artificial intelligence (i.e., machine learning, deep learning, and reinforcement learning) in MEC-assisted video streaming services.

==> figures/forest.tex <==

% \newcolumntype{C}[1]{>{\centering}p{#1}}
% \begin{forest}
% % forked edges,
% % for tree={grow=east, 
% %             anchor=center, 
% %             draw=gray, fill=color1, 
% %             align=center, inner sep=5pt,
% %             l sep-=0,l=0,
% %             child anchor=west, parent anchor=east,
% %             % grow'=east, anchor=west,
% %             %text width=2cm, minimum height=1cm,
% %             drop shadow},

% for tree={
%   if level=0{align=center}{% allow multi-line text and set alignment
%     align={@{}C{45mm}@{}},
%   },
%   grow=east,
%   draw,
%   font=\sffamily\bfseries,
%   edge path={
%     \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) -- +(5mm,0) |- (.child anchor)\forestoption{edge label};
%   },
%   parent anchor=east,
%   child anchor=west,
%   l sep=10mm,
%   tier/.wrap pgfmath arg={tier #1}{level()},
%   edge={ultra thick, rounded corners=2pt},
%   fill=white,
%   rounded corners=2pt,
%   drop shadow,
% },


% [\textbf{Resource Allocation}


% [Single User \small{(single dedicated server)}
%     [Deterministic
%         [Binary offloading]
%         [Partial offloading]]
%     [Stochastic]
% ]
    
% [Multi User \small{(one shared server)}
%     [Server scheduling [Scheduling A][Scheduling B]]
%     [Joint resource allocation [Joint radio and caching][Joint radio and transcoding]]
% ]    
    
% [Multi Server \small{(multiple shared servers)}
%     [Server selection] 
%     [Server cooperation [One-hop neighbors] [client-server path] [Edge cloud cooperation]] 
%     [Computation migration]
% ]


% ]
% \end{forest}




% % \begin{tikzpicture}[
% % node1/.style={rectangle, draw=gray!80, fill=color1, very thick, minimum width=3cm, minimum height=1cm},
% % node2/.style={rectangle, draw=gray!80, fill=color1, very thick, minimum width=2.5cm, minimum height=1cm, yshift=-1cm},
% % node3/.style={rectangle, draw=gray!80, fill=color1, very thick, minimum width=3cm, minimum height=0.8cm, yshift=-1cm},]

% % \node[node1] (r) {Resource Allocation};

% % \node[node2] (a1) [below of=r, xshift=-6cm] {Single user};
% % \node[node2] (a2) [below of=r, xshift=0] {Multi user};
% % \node[node2] (a3) [below of=r, xshift=6cm] {Multi Server};


% % \node[node2] (b1) [below of=a1, xshift=-2cm] {Deterministic};
% % \node[node2] (b2) [below of=a1, xshift=2cm] {Stochastic};

% % \node[node3] (b11) [below of=b1, xshift=-1cm] {Binary offloading};
% % \node[node3] (b12) [below of=b1, xshift=1cm] {Partial Offloading};


% % % Lines
% % \draw[-] (r.south) |- (a1.north);
% % \draw[-] (r.south) |- (a2.north);
% % \draw[-] (r.south) |- (a3.north);
% % \end{tikzpicture}


\newcolumntype{C}[1]{>{\centering}p{#1}}
\begin{forest}
for tree={
  if level=0{align=center}{% allow multi-line text and set alignment
    align={@{}C{30mm}@{}},
  },
  grow=east,
  draw,
%   font=\sffamily\bfseries,
  font=\small,
  edge path={
    \noexpand\path [draw, color=gray, \forestoption{edge}] (!u.parent anchor) -- +(5mm,0) |- (.child anchor)\forestoption{edge label};
  },
  parent anchor=east,
  child anchor=west,
  l sep=10mm,
  tier/.wrap pgfmath arg={tier #1}{level()},
  edge={ultra thick, rounded corners=2pt, color=gray},
  fill=white,%fill color
  rounded corners=2pt,
  drop shadow,
}
[Computation Offloading
  [Single User System
    [Deterministic Task Arrival
        [Binary offloading]
        [Partial offloading]
    ]
    [Stochastic Task Arrival
        [Dynamic offloading policies]
    ]
  ]
  [Multi User System
  [Server Scheduling]
  [Joint Resource Allocation
        [Joint Radio and Caching]
        [Joint Radio and Transcoding]
    ]
    [Multi User Scheduling]
    ]
    [Multi Server System
    [Server Selection]
    [Server Cooperation
        [Single Hop]
        [Delivery Path]
        [Cloud-Edge]
    ]
    [Computational Migration]
    ]
]
\end{forest}


==> tables/cache_replace.tex <==
LRU &Replace least recently used (older) contents. \\[1em]
R-UPP \cite{ahlehagh_2014} &Replace videos based on user preferences profiles (UPP) of active users. \\[1em]
WDDQN \cite{li_2020} &Cache replacement policy by offloading contents to mobile users via D2D communication. \\[1em]

==> tables/caching.tex <==

\begin{tabular}{p{2cm} p{0.5cm} p{1.5cm} p{10cm}}
\toprule[1pt] 

\textbf{Category} &\textbf{Ref} &\textbf{Scheme} &\textbf{Description} \\
\midrule

\multirow{5}{*}{Content Fetching} 
& [X] & MPV &Using nation-wide popularity. \\

& \cite{ahlehagh_2014} &P-UPP  &Predict and cache videos most probably to be requested by active users. \\

&\cite{gharaibeh_2016} &Scheme &Proactively fetch contents (without knowing popularity) to reduce the sum of storage cost and user attrition cost. \\

&\cite{tran_2017} & JCCP  &Jointly optimize caching and transcoding resources using ILP to minimize the backhaul network cost. \\

&\cite{bilal_2019} &CJCT  &Profetch contents from neighboring servers using X2 backhaul interrface or fetch highest bitrate version of the video from CDN server. \\[2em]
\midrule \midrule

%%% Cache Replacement
\multirow{3}{*}{Cache Replacement} 
&[X] &LRU &Replace least recently used (older) contents. \\

&\cite{ahlehagh_2014} &R-UPP  &Replace videos based on user preferences profiles (UPP) of active users. \\

&\cite{li_2020} &WDDQN &Cache replacement policy by offloading contents to mobile users via D2D communication. \\






\bottomrule[1pt]
\end{tabular}

==> tables/mec_stream.tex <==


\begin{tabular}{p{3cm} p{4cm}}\toprule
Category &Ref \\\midrule
% [1] [4] [13] [19] [20] [28] [41] [66] [70]
Edge based caching & \cite{Ahlehagh2014a, Su2017, Vigneri2019, Yang2019, Qu2020, Wang2019b, Zhang2020a, Cheng2020, Kumar2020} \\

%[9] [74]
Edge based transcoding 
&\cite{Wang2019d, Feng2020a} \\

% [6] [16] [36] [44] [47] [61] [65]
Proactive caching 
&\cite{Ge2017, Tran2019, Han2020, Li2020a, Tran2020, Baccour2020, Zeng2019} \\

% [23] [28] [51] [64] [69]
Cooperative caching 
&\cite{Jiang2019, Wang2019b, Rezvani2018, Chien2020a, Bilal2019} \\

% [40] [51]
Cooperative processing/computing 
&\cite{Sun2020, Rezvani2018} \\

% [8] [12] [16] [25] [31] [34] [48] [51] [61] [69] [71]
Joint caching and computing 
& \cite{Yang2018a, Yan2019, Tran2019, Hao2019, Xie2019, Tang2019, Zhang2020b, Rezvani2018, Baccour2020, Bilal2019, Zhang2020} \\

Joint radio and computing 
& \\

% [24] [27] [37] [45]
Joint radio, caching and computing 
& \cite{Dang2019, Sun2019, Luo2019, Wang2020h} \\

% [2] [11] [14] [15] [32] [33] [37] [38] [44] [47] [56]
Edge enabled adaptive streaming and bitrate selection 
& \cite{Yan2017, Mehrabi2019a, Liang2018, Mehrabi2018, Wang2020c, Rahman2019, Luo2019, Lu2020, Li2020a, Tran2020, Seufert2015} \\

% [3]
Predicting users requests pattern 
& \cite{Ma2017} \\
\bottomrule
\end{tabular}

==> tables/mec_stream_soa2.tex <==

% \rowcolors{2}{}{gray!15}
% \begin{tabular}{|w|g|g|g|g|g|}
\begin{tabular}{|m{2cm}|m{0.5cm}|m{13cm}|m{3cm}|}
\hline 
Category &Ref &Description of Contribution & QoS Metric\\[0.5em] \hline \hline

%%%%%%%%%%%%  Caching

%% Caching and Proactive Content Fetching
\multirow{9}{2cm}{Caching and Proactive Content Fetching} 
&\cite{ahlehagh_2014} &Fetch Most Popular Videos (MPV) using nation-wide popularity. &\khan{Capacity} \\ \cline{2-4}
&\cite{gharaibeh_2016}  &Proactively fetch contents to reduce the sum of storage cost and user attrition cost. &\khan{Network cost} \\\cline{2-4}
&\cite{Tran2020} & Caching based on popularity and retention rate of video streams to maximize their video bitrate. &\khan{Video bitrate} \\\cline{2-4}
&\cite{Zeng2019} & Smart caching based on user behavior to maximize the hit rate of contents within limited time. &\khan{Cache hit rate} \\\cline{2-4}
&\cite{Su2017} & Cache layered videos for multiple user groups. Users in same group share caching cost. &\khan{Hit ratio, delay} \\\cline{2-4}
&\cite{Yang2019} & Prefetch popular videos from YouTube using ML-based prediction. &\khan{Hit ratio, Freeze count, throughput} \\\cline{2-4}
&\cite{Kumar2020} & Cache videos that serves the maximum number of users by estimating the probability distribution of requested video qualities using RAN status information. &\khan{Capacity, hit ratio, delay} \\\cline{2-4}
& \khan{\cite{yang2021_2}} & \khan{Edge caching strategy for vehicular networks in which video content is stored on the RSU and fetched by vehicular users.} &\khan{Hit ratio, latency} \\ [0.0em]  \hline \hline
% \cline{2-4}


%% Cooperative Caching 
\multirow{18}{2cm}{Cooperative Caching}
&\cite{bilal_2019} & Prefetch highest bitrate version of the video from CDN server using X2 interface. &\khan{Network cost, delay, cache hit ratio} \\\cline{2-4}
&\cite{Vigneri2019} & Prefetch video chunks into their playout buffer from encountered vehicle caches and stream from the cellular infrastructure when their playout buffer empties. &\khan{offloading gain} \\\cline{2-4}
&\cite{Qu2020} & Solve the multiple bitrate video caching problem using polynomial complexity algorithm. &\khan{QoE function} \\\cline{2-4}
&\cite{Zhang2020a} & Operators advertise contents to attract a mobile user to request cached contents at the edge instead of non-cached contents. &\khan{Benefit to content providers} \\\cline{2-4}
&\cite{Cheng2020} & Context-aware adaptive caching through network virtualization at the edge. &\khan{Total energy consumption} \\\cline{2-4}
&\cite{Li2020a} & Jointly optimize caching of bitrate-aware files and the scheduling of video requests to minimize the total expected energy consumption. &\khan{Energy consumption, cache hit ratio} \\\cline{2-4}

% As before [23] [28] [51] [64] [69]
& \cite{tran_2017} &Jointly optimize caching and transcoding resources using ILP to minimize the backhaul network cost. &\khan{Cache hit ratio, access delay, network cost} \\\cline{2-4}
&\cite{Jiang2019} & Cooperative caching when users' preference is unknown and only the historical content demands. &\khan{Cache hit ratio, delay} \\\cline{2-4}
&\cite{Wang2019b} & Joint caching placement (long-term) and video retrieval (short-term) in coordinated multi-server system. &\khan{Access delay, cache hit ratio} \\\cline{2-4}
&\cite{Chien2020a} & Using Q-learning, find the appropriate cache state to improve caching mechanism. &\khan{A}\\\cline{2-4}
%% Copied from Caching
&\cite{Tran2019} & Joint collaborative caching video requests and processing requests at multiple servers to minimize the expected delay cost of video retrieval. &\khan{Cache hit ratio, access delay, network cost} \\ \cline{2-4}
&\cite{Baccour2020} & A joint caching and processing model to proactively cache only the chunks of videos to be watched with collaboration among neighboring MECs to further improve storage utilization. &\khan{Network cost, average delay and cache hit ratio} \\\cline{2-4}
&\khan{\cite{sang2021}} & \khan{A greedy collaborative caching strategy in heterogenous MEC network to minimize the total delay costs of all users.}. &\khan{Cache hit ratio, average delay, network load} 
\\[0.8em]  \hline \hline


%%%%%%%%%%%% Transcoding
%% Edge-based transcoding [40] [51] 
\multirow{2}{2cm}{Cooperative Processing} 
&\cite{Sun2020} &Edge nodes pre-process video data using a lightweight DNN model and upload the results to cloud nodes for further analysis. &\khan{Energy consumption, delay} \\\cline{2-4}
&\khan{\cite{taha2021}} &\khan{A QoS-aware method to implement peer-offloading using perceptual parameters such as pausing frequency, watching percentage and bit rates.} &\khan{Perceptual and systemic QoE}   \\[0.8em]  \hline \hline
% \cline{2-4}

%% Joint caching and computing [8] [12] [16] [25] [31] [34] [48] [51] [61] [69] [71]
\multirow{16}{2cm}{Joint Caching and Processing} 
% & \cite{tran_2017} &Jointly optimize caching and transcoding resources using ILP to minimize the backhaul network cost. &\khan{A} \\
&\cite{Yang2018a} &Reduce communication-resource consumption by using MEC to select and compute components not stored on VR device. &\khan{Communication Cost}  \\\cline{2-4}
&\cite{Yan2019} &Implement per-channel optimal service-aware resource allocation. &\khan{Playback rate, buffer level} \\\cline{2-4}
&\cite{Tran2019} &A low-complexity online request scheduling algorithm to decide whether to transcod locally or to search a transcodable variant from other neighboring caches or fetch from the origin content server. &\khan{Cache hit ratio, access delay, network cost} \\\cline{2-4}
&\cite{Hao2019} &A video caching and processing model that offers maximized profit to video service provider. &\khan{Content provider's profit} \\\cline{2-4}
&\cite{Xie2019} &A joint caching and transcoding schedule strategy for HTTP adaptive video to minimize the system energy consumption. &\khan{Energy consumption} \\\cline{2-4}
&\cite{Tang2019} &BSs compete to maximise its revenue by maximising the request rate that can be served by the MEC server. &\khan{Utilization of storage and computational resources} \\\cline{2-4}
&\cite{Zhang2020b} &to minimize the average retrieval latency of all users using greedy rounding proactively caching and random-rounding user-BS association scheme. &\khan{Delay, hit ratio, backhaul traffic} \\\cline{2-4}
&\cite{Baccour2020} & A joint caching and processing model to proactively cache only the chunks of videos to be watched instead of caching the whole video content. Collaboration among neighboring MECs improves storage utilization. &\khan{Network cost, average delay and cache hit ratio} \\\cline{2-4}
&\cite{Bilal2019} &Online bit rate conversion to the requested version of videos fetched from the origin/CDN servers. &\khan{Network cost, average delay, hit ratio} \\\cline{2-4}
&\cite{Zhang2020} &Joint task offloading and dynamic caching strategy to reduce overall latency of all mobile devices.  &\khan{Energy, service latency} \\\cline{2-4}
&\khan{\cite{huang2021}} & \khan{Joint optimization of caching and transcoding for resource allocation in DASH.} &\khan{Throughput, hit ratio, rebuffering delay} \\[0.8em]  \hline \hline
% \cline{2-4}

%% Joint radio, caching and computing [24] [27] [37] [45]
\multirow{10}{2cm}{Joint Radio, Caching and Processing} 
&\cite{Dang2019} &Joint radio, caching and computing scheme to maximize the average tolerant delay with meeting a given transmission rate constraint in VR devices. &\khan{Average delay}  \\\cline{2-4}
&\cite{Sun2019} &A mobile VR delivery framework to decide whether to pre-cache (and if yes, which) parts of the field of views (FOVs), with some pre-processing on mobile. &\khan{Communication bandwidth}  \\\cline{2-4}
&\cite{Luo2019} &Jointly consider buffer dynamics, video quality adaption, edge caching, video transcoding and transmission for energy saving and QoE enhancement. &\khan{Energy saving} \\\cline{2-4}
&\cite{Wang2020h} &Jointly optimize the caching decision
and radio and computation resource allocation to maximize the system revenue. &\khan{Revenue} \\
&\cite{Rezvani2018} & Joint multi-bitrate video caching and transcoding by allocating physical and radio resources based on network stochastic information.  &\khan{Revenue} \\\cline{2-4}
&\khan{\cite{cheng2021}} & \khan{Jointly considers data transmission, video coding, caching, and computation to meet the delay requirement in mobile VR video streaming.}.  &\khan{End to End delay} \\\cline{2-4}
&\khan{\cite{liu2021}} & \khan{Jointly optimize cachig, processing and transmission to reduce latency}. &\khan{Latency}  \\[0.8em]  \hline




%%%%%%%%%%%% Adaptive Bit Streaming
% \multirow{4}{2cm}{Edge enabled adaptive streaming}

% %% Category 1
% &\multirow{2}{2cm}{Category 1} 
% &5 &ABC \\
% & &6 &ABC \\ 
% \cmidrule{2-4}

% %% Category 2
% &\multirow{2}{2cm}{Category 2} 
% &7 &ABC \\
% & &8 &ABC \\




%%%% End Tablular
\end{tabular}





==> tables/resource_alloc.tex <==
% \rowcolors{2}{gray!15}{white}
\rowcolors{2}{}{gray!15}
\begin{tabular}{| m{2cm} | m{0.5cm} | m{8cm} | m{2.5cm} | m{2.5cm} |}
% \begin{tabular}{| m{2cm} | g|g|g|g}
\hline
Category  &Ref &Description &\khan{Evaluation Metrics} & \khan{Method/Algorithm}\\[0.5em] \hline \hline
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3}
% \arrayrulecolor{white}



% Binary offloading
\multirow{4}{2cm}{Binary Offloading}
& \cite{barbarossa_2014} & Transmission energy minimization under computation deadline. &\khan{Delay, Energy}  &\khan{Convex programming}\\ \cline{2-5}
& \cite{zhang_2013} & Minimize energy consumption with a soft real-time requirement. &\khan{Delay, Energy}  &\khan{Convex Programming}\\
& \cite{Hao2019} & A binary offloading model to maximize profit to video service provider. &\khan{N/A} &\khan{MAB}
\\[1.5em] \hline

% Partial Offloading
\multirow{4}{2cm}{Partial Offloading} 
& \cite{wei_2018} & Schedule offloading tasks from multiple mobile nodes to a single MEC server in order to maximize energy savings of all mobile nodes. &\khan{Energy}  &\khan{SMSEF}\\ 
& \cite{wang_2016} & Task-input data is divided for local and remote execution. &\khan{Energy, Latency}  &\khan{uni-variate search}\\ 
& \cite{jia_2014} & Load balancing between mobile and edge servers to minimize latency. &\khan{Latency}  &\khan{Heuristic}
\\[1.5em] \hline

% Stochastic Offloading
\multirow{3}{2cm}{Stochastic Offloading} 
& \cite{yang_2018} & Reinforcement learning to proactive allocation resources to multiple. &\khan{E2E Reliability}  &\khan{Q-learning}\\ 
& \cite{haouari_2019_2} & Transcoding resource allocation using past video requests and then using time series forecasting to predict the resources needed for future requests using a heuristic. &\khan{QoE, Network cost}  &\khan{LSTM, GRU, CNN, MLP, XGboost}
\\[1.5em] \hline


% Server Scheduling
\multirow{4}{2cm}{Server Scheduling} 
& \cite{mehrabi_2019} & A scheduling algorithm that solves client to edge mapping (load balancing) and per client bit rate selection problems. &\khan{Throughput, Buffer delay, Fairness}  &\khan{Heuristic} \\
& \cite{molina_2014} & Scheduling uplink and downlink transmissions using queuing theory. &\khan{Energy}  &\khan{Nested interval algorithm}\\  
& \cite{guo_2016} & Tasks Offloading selection using clock frequency and transmission power allocation. &\khan{Energy, Delay}  &\khan{DVFS}
\\[1.5em] \hline

% Joint Radio and Processing
\multirow{2}{2cm}{Joint Radio and Processing} 
& \cite{ren_2019} & Jointly optimize communication and computational resources with tasks splitting between edge and cloud. &\khan{Latency}  &\khan{Convex optimization}\\ 
& \cite{barbarossa_2013} & Joint allocation of computation and radio resources. &\khan{Power consumption}  &\khan{Convex optimization}
\\[1.5em] \hline


% Joint Caching and Processing 
\multirow{4}{2cm}{Joint Caching and Processing} 
& \cite{tran_2017} & Jointly optimize caching and transcoding resources to minimize the backhaul network cost. &\khan{Network cost}  &\khan{ILP} \\
&\cite{Ge2017} & Collaborative offloading and caching scheme using Lyapunov optimization to minimize the overall latency of all mobile devices. &\khan{Throughput, Playout delay, Buffer length, Rebuffering duration}  &\khan{Theoretical architecture}
\\[1.5em] \hline


% Server Selection
\multirow{5}{2cm}{Server Selection} 
& \cite{niu_2019} & Balance work load among edge nodes by considering edge computing capability, existing work load and distance among edge server and user. &\khan{Service delay}  &\khan{PSO}\\ 
& \cite{haouari_2019} & Proactively allocate resources by predicting the number of viewers in a cloud site and then serving viewers by their closest server. &\khan{Viewers' QoE, Network cost}  &\khan{MLP, DT, RF}
\\[1.5em] \hline


% Server Cooperation
\multirow{5}{2cm}{Server Cooperation} 
& \cite{bilal_2019} & edge servers in a sing-hop clusters cooperate to cache and transcode contents. &\khan{Network cost, delay, cache hit ratio}  &\khan{ILP}\\  
& \cite{ren_2019} & Jointly optimize communication and computational resources with tasks splitting between edge and cloud. &\khan{Delay}  &\khan{Convex optimization}\\  
& \cite{zhao_2015} & Edge/cloud selection to meet deadline requirements. &\khan{Task completion}  &\khan{Heuristic}
\\[1.5em] \hline


% Server Migration
\multirow{6}{2cm}{Computation Migration} 
& \cite{wang_2014} &Computation migration based on distance threshold between user and two servers using MDP. &\khan{MDP}  &\khan{Delay}\\ 
& \cite{urgaonkar_2015} & Jointly optimize computation scheduling and service migration to minimize energy transmission and reconfiguration cost. &\khan{MDP}  &\khan{Application queue length} \\  
& \cite{chen_2016} & Compute locally or offload to remote server such that total energy consumption and latency is minimized. &\khan{Energy, Delay}  &\khan{MIP}
\\[1.5em] \hline
\end{tabular}



==> tables/surveys.tex <==

   \begin{tabular}{p{2cm} p{5cm}}
   \toprule
    Ref   & Contribution \\
    \midrule
    
    %% Generic
    \cite{cao_2020, lin_2020, shakarami_2020, de_2019, khan_2019, hassan_2019, abbas_2018, wang_2017, baktir_2017, ahmed_2017, taleb_2017, mao_2017, ahmed_2016, shi_2016} 
    & Generic (covers multiple topics including architecture, use cases, benefits and challenges etc.) \\[1.5em]
    
    %% Offloading
    \cite{prerna_2020, jiang_2019, lin_2019} 
    & Computation offloading in edge computing  \\[1.5em]
    
    %% Communication
    \cite{mao_2017_2} 
    & Communication in edge computing  \\[1.5em]
    
    %% Security
    \cite{xiao_2019, yang_2019, liu_2019, zhang_2018, roman_2018, shirazi_2017}
    & Security in Mobile Edge Computing \\[1.5em]
    
    %% IoT
    \cite{marjanovic_2018, porambage_2018,yu_2017} 
    & Internet of Things (IoT) and Crowdsensing  \\[1.5em]
    
    
    %% ML, DL, AI
    \cite{wang_2020, deng_2020, shakarami_2020, carvalho_2020, chen_2019} 
    & Deep Learning for edge computing  \\[1.5em]
    
    %% This survey
    This survey
    & Explains the State-of-the-art in mobile edge computing in video streaming services, covering challenges and opportunities. Dedicated sections on using device-to-device cooperation and novel deep learning techniques are provided.\\
    
    
    
    \bottomrule
    \end{tabular}
